Joint Metrics Matter: A Better Standard for Trajectory Forecasting

Multi-modal trajectory forecasting methods commonly evaluate using single-agent metrics (marginal metrics), such as minimum Average Displacement Error (ADE) and Final Displacement Error (FDE), which fail to capture joint performance of multiple interacting agents. Only focusing on marginal metrics can lead to unnatural predictions, such as colliding trajectories or diverging trajectories for people who are clearly walking together as a group. Consequently, methods optimized for marginal metrics lead to overly-optimistic estimations of performance, which is detrimental to progress in trajectory forecasting research. In response to the limitations of marginal metrics, we present the first comprehensive evaluation of state-of-the-art (SOTA) trajectory forecasting methods with respect to multi-agent metrics (joint metrics): JADE, JFDE, and collision rate. We demonstrate the importance of joint metrics as opposed to marginal metrics with quantitative evidence and qualitative examples drawn from the ETH / UCY and Stanford Drone datasets. We introduce a new loss function incorporating joint metrics that, when applied to a SOTA trajectory forecasting method, achieves a 7\% improvement in JADE / JFDE on the ETH / UCY datasets with respect to the previous SOTA. Our results also indicate that optimizing for joint metrics naturally leads to an improvement in interaction modeling, as evidenced by a 16\% decrease in mean collision rate on the ETH / UCY datasets with respect to the previous SOTA. Code is available at \texttt{\hyperlink{https://github.com/ericaweng/joint-metrics-matter}{github.com/ericaweng/joint-metrics-matter}}.

==> tables/all_vvs.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{}
\label{table:eth_ucy_min_JADE_min_JFDE}
\subfloat[\textit{JADE} / \textit{JFDE}]{
\label{table:eth_ucy_min_JADE_min_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.919 / 1.742 & 0.480 / 0.950 & 0.744 / 1.573 & 0.438 / 1.001 & 0.362 / 0.794 & 0.589 / 1.212\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.726 / 1.299 & 0.237 / 0.418 & 0.609 / 1.316 & 0.359 / 0.712 & 0.294 / 0.625 & 0.445 / 0.874\\
PECNet \cite{mangalam2020not} & 0.618 / 1.097 & 0.291 / 0.587 & 0.666 / 1.417 & 0.408 / 0.896 & 0.372 / 0.840 & 0.471 / 0.967\\
Y-Net no scene \cite{mangalam_goals_2020} & 0.479 / 0.785 & 0.215 / 0.423 & - / - & 0.401 / 0.867 & 0.318 / 0.680 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.495 / 0.781 & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974\\
Y-Net ped \cite{mangalam_goals_2020} & 0.486 / 0.784 & 0.293 / 0.610 & 33.918 / 73.481 & 0.407 / 0.718 & 0.332 / 0.704 & 7.087 / 15.260\\
Y-Net old \cite{mangalam_goals_2020} & 0.489 / 0.868 & 0.230 / 0.413 & - / - & 0.377 / 0.785 & 0.336 / 0.717 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.495 / 0.781 & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974\\
MemoNet \cite{Xu2022-ki} & 0.499 / 0.859 & 0.222 / 0.416 & 0.686 / 1.466 & 0.349 / 0.723 & 0.385 / 0.864 & 0.428 / 0.866\\
View Vertically \cite{Wong2022-kx} & 0.561 / 0.776 & 0.196 / 0.332 & 0.654 / 1.307 & 0.328 / 0.654 & 0.298 / 0.602 & 0.408 / 0.734\\
View Vertically w/ joint loss (Ours) & 0.651 / 0.924 & 0.182 / 0.303 & 0.628 / 1.263 & 0.334 / 0.645 & 0.269 / 0.544 & 0.413 / 0.736\\
vv a 0.2-0.8 b 0.3-0.5-0.2 & 0.631 / 0.803 & - / - & - / - & - / - & - / - & - / -\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.202 / 0.326 & 0.602 / 1.233 & 0.332 / 0.657 & 0.263 / 0.529 & - / -\\
vv a 0.2,0.8 b 0.3,0.5,0.2 & 0.630 / 0.808 & 0.194 / 0.302 & 0.649 / 1.293 & 0.329 / 0.624 & 0.263 / 0.536 & 0.413 / 0.712\\
vv a 0.7,0.3 b 0.5,0.3,0.2 & 0.722 / 0.921 & \underline{0.177} / 0.285 & 0.583 / 1.202 & 0.331 / 0.637 & 0.270 / 0.542 & 0.417 / 0.718\\
vv a 0.8,0.2 b 0.6,0.2,0.2 & 0.683 / 0.947 & 0.196 / 0.309 & 0.591 / 1.214 & 0.334 / 0.662 & 0.269 / 0.543 & 0.415 / 0.735\\
vv a 0.8,0.2 b 0.5,0.3,0.2 & 0.687 / 0.951 & 0.194 / 0.301 & 0.593 / 1.216 & 0.333 / 0.663 & 0.269 / 0.542 & 0.415 / 0.735\\
vv a 0.8,0.2 b 0.4,0.4,0.2 & 0.686 / 0.953 & 0.196 / 0.308 & 0.593 / 1.217 & 0.336 / 0.661 & 0.269 / 0.543 & 0.416 / 0.736\\
vv a 0.7,0.3 b 0.6,0.2,0.2 & 0.734 / 0.950 & \textbf{0.176} / \underline{0.280} & 0.600 / 1.220 & 0.330 / 0.633 & 0.270 / 0.544 & 0.422 / 0.725\\
vv a 0.7,0.3 b 0.4,0.4,0.2 & 0.722 / 0.941 & 0.177 / \textbf{0.279} & 0.600 / 1.219 & 0.331 / 0.634 & 0.270 / 0.543 & 0.420 / 0.723\\
vv a 0.6,0.4 b 0.5,0.3,0.2 & 0.694 / 0.907 & 0.200 / 0.327 & 0.567 / 1.148 & 0.324 / 0.630 & 0.270 / 0.541 & 0.411 / 0.711\\
vv a 0.6,0.4 b 0.4,0.4,0.2 & 0.695 / 0.903 & 0.201 / 0.331 & \underline{0.566} / \underline{1.148} & 0.324 / 0.629 & 0.269 / 0.539 & 0.411 / 0.710\\
vv a 0.5,0.5 b 0.4,0.4,0.2 & 0.650 / 0.858 & 0.187 / 0.315 & 0.578 / 1.202 & 0.333 / 0.635 & 0.266 / 0.547 & 0.403 / 0.711\\
vv a 0.5,0.5 b 0.5,0.3,0.2 & 0.652 / 0.839 & 0.186 / 0.309 & \textbf{0.523} / \textbf{1.091} & 0.331 / 0.634 & 0.267 / 0.547 & 0.392 / 0.684\\
vv a 0.5,0.5 b 0.6,0.2,0.2 & 0.653 / 0.848 & 0.186 / 0.313 & 0.584 / 1.212 & 0.334 / 0.636 & 0.267 / 0.546 & 0.405 / 0.711\\
AgentFormer \cite{yuan_agentformer_2021} & 0.482 / 0.794 & 0.237 / 0.456 & 0.622 / 1.310 & 0.285 / 0.564 & 0.296 / 0.624 & 0.384 / 0.749\\
\textbf{Joint AgentFormer (Ours)} & 0.485 / 0.798 & 0.186 / 0.320 & 0.590 / 1.219 & \underline{0.271} / \underline{0.513} & 0.252 / 0.509 & \textbf{0.357} / \textbf{0.672}\\
ablation 7.5 & \underline{0.477} / \textbf{0.747} & 0.191 / 0.335 & 0.609 / 1.262 & 0.272 / 0.524 & \underline{0.248} / \underline{0.502} & 0.360 / 0.674\\
\textbf{Joint AgentFormer (old)} & 0.486 / 0.780 & 0.194 / 0.338 & 0.602 / 1.246 & \textbf{0.267} / \textbf{0.513} & \textbf{0.242} / \textbf{0.482} & \underline{0.358} / \underline{0.672}\\
ablation 10 & \textbf{0.465} / \underline{0.755} & 0.193 / 0.334 & 0.608 / 1.256 & 0.273 / 0.529 & 0.260 / 0.525 & 0.360 / 0.680\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\subfloat[$CR_{JADE}$ / $CR_{mean}$]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\text{CR}_{JADE} / \text{CR}_{mean} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.021 / 0.015 & 0.025 / 0.031 & 0.165 / 0.165 & 0.057 / 0.060 & 0.074 / 0.083 & 0.068 / 0.071\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.031 / 0.025 & 0.038 / 0.044 & 0.267 / 0.281 & 0.083 / 0.088 & 0.092 / 0.126 & 0.102 / 0.113\\
PECNet \cite{mangalam2020not} & 0.009 / 0.014 & 0.037 / 0.043 & 0.211 / 0.218 & 0.050 / 0.059 & 0.112 / 0.128 & 0.084 / 0.092\\
Y-Net no scene \cite{mangalam_goals_2020} & 0.044 / 0.062 & 0.023 / 0.075 & - / - & 0.051 / 0.114 & 0.073 / 0.141 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.028 / 0.016 & 0.030 / 0.039 & 0.209 / 0.265 & 0.065 / 0.100 & 0.097 / 0.134 & 0.086 / 0.111\\
Y-Net ped \cite{mangalam_goals_2020} & 0.019 / 0.016 & 0.042 / 0.044 & \textbf{0.005} / \textbf{0.007} & 0.039 / 0.068 & 0.072 / 0.098 & \textbf{0.035} / \textbf{0.047}\\
Y-Net old \cite{mangalam_goals_2020} & 0.071 / 0.062 & 0.035 / 0.073 & - / - & 0.058 / 0.104 & 0.087 / 0.120 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.028 / 0.016 & 0.030 / 0.039 & 0.209 / 0.265 & 0.065 / 0.100 & 0.097 / 0.134 & 0.086 / 0.111\\
MemoNet \cite{Xu2022-ki} & 0.031 / 0.014 & 0.034 / 0.040 & 0.192 / 0.206 & 0.060 / 0.065 & 0.119 / 0.136 & 0.087 / 0.092\\
View Vertically \cite{Wong2022-kx} & 0.012 / 0.014 & 0.020 / 0.029 & 0.187 / 0.212 & 0.034 / 0.045 & 0.059 / 0.082 & 0.062 / 0.077\\
View Vertically w/ joint loss (Ours) & 0.023 / 0.015 & 0.024 / 0.032 & 0.187 / 0.216 & 0.030 / 0.050 & 0.058 / 0.075 & 0.064 / 0.077\\
vv a 0.2-0.8 b 0.3-0.5-0.2 & 0.006 / 0.011 & - / - & - / - & - / - & - / - & - / -\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.021 / 0.035 & 0.174 / 0.213 & 0.032 / 0.043 & 0.053 / 0.077 & - / -\\
vv a 0.2,0.8 b 0.3,0.5,0.2 & 0.017 / 0.011 & \underline{0.006} / 0.028 & 0.171 / 0.216 & 0.035 / 0.038 & 0.052 / 0.071 & 0.056 / 0.073\\
vv a 0.7,0.3 b 0.5,0.3,0.2 & 0.021 / 0.014 & 0.017 / 0.025 & 0.375 / 0.364 & 0.037 / 0.040 & 0.053 / 0.075 & 0.100 / 0.104\\
vv a 0.8,0.2 b 0.6,0.2,0.2 & 0.009 / 0.014 & 0.019 / 0.021 & 0.171 / 0.199 & 0.032 / 0.037 & 0.054 / 0.075 & 0.057 / 0.069\\
vv a 0.8,0.2 b 0.5,0.3,0.2 & 0.019 / 0.015 & 0.019 / 0.026 & 0.175 / 0.199 & 0.033 / 0.036 & 0.054 / 0.074 & 0.060 / 0.070\\
vv a 0.8,0.2 b 0.4,0.4,0.2 & 0.009 / 0.013 & 0.018 / 0.023 & 0.173 / 0.200 & 0.032 / 0.037 & 0.054 / 0.074 & 0.057 / 0.069\\
vv a 0.7,0.3 b 0.6,0.2,0.2 & 0.016 / 0.014 & 0.013 / 0.026 & 0.176 / 0.191 & 0.034 / 0.039 & 0.050 / 0.075 & 0.058 / 0.069\\
vv a 0.7,0.3 b 0.4,0.4,0.2 & 0.017 / 0.014 & 0.013 / 0.025 & 0.178 / 0.190 & 0.035 / 0.040 & 0.052 / 0.075 & 0.059 / 0.069\\
vv a 0.6,0.4 b 0.5,0.3,0.2 & 0.007 / \underline{0.010} & 0.020 / 0.027 & 0.202 / 0.238 & 0.024 / 0.040 & 0.064 / 0.079 & 0.063 / 0.079\\
vv a 0.6,0.4 b 0.4,0.4,0.2 & 0.012 / \textbf{0.009} & 0.016 / 0.027 & 0.203 / 0.240 & 0.028 / 0.041 & 0.059 / 0.080 & 0.064 / 0.079\\
vv a 0.5,0.5 b 0.4,0.4,0.2 & 0.009 / 0.011 & 0.027 / 0.025 & 0.350 / 0.399 & 0.026 / 0.045 & 0.059 / 0.080 & 0.094 / 0.112\\
vv a 0.5,0.5 b 0.5,0.3,0.2 & \underline{0.005} / 0.011 & 0.026 / 0.026 & 0.236 / 0.276 & 0.026 / 0.045 & 0.059 / 0.081 & 0.070 / 0.088\\
vv a 0.5,0.5 b 0.6,0.2,0.2 & \textbf{0.005} / 0.011 & 0.019 / 0.026 & 0.346 / 0.397 & 0.027 / 0.044 & 0.060 / 0.080 & 0.091 / 0.112\\
AgentFormer \cite{yuan_agentformer_2021} & 0.012 / 0.016 & 0.019 / 0.022 & 0.182 / 0.204 & \underline{0.014} / 0.021 & 0.048 / \underline{0.054} & 0.055 / 0.063\\
\textbf{Joint AgentFormer (Ours)} & 0.017 / 0.013 & 0.011 / 0.019 & 0.159 / 0.163 & 0.015 / 0.021 & \underline{0.041} / 0.055 & 0.049 / 0.054\\
ablation 7.5 & 0.015 / 0.012 & \textbf{0.006} / 0.019 & \underline{0.149} / \underline{0.154} & \textbf{0.012} / \textbf{0.020} & 0.044 / 0.056 & \underline{0.045} / \underline{0.052}\\
\textbf{Joint AgentFormer (old)} & 0.013 / 0.012 & 0.010 / \textbf{0.016} & 0.150 / 0.163 & 0.018 / 0.020 & \textbf{0.037} / \textbf{0.054} & 0.046 / 0.053\\
ablation 10 & 0.021 / 0.014 & 0.007 / \underline{0.017} & 0.153 / 0.163 & 0.015 / \underline{0.020} & 0.045 / 0.060 & 0.048 / 0.055\\
\hline
Ground Truth & 0.000 & 0.001 & 0.021 & 0.000 & 0.002 & 0.005\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_ADE_min_FDE}
\subfloat[\ADE / \FDE]{
\label{table:eth_ucy_min_ADE_min_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{ADE}_{20} / \text{FDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.876 / 1.656 & 0.461 / 0.920 & 0.639 / 1.343 & 0.379 / 0.816 & 0.285 / 0.600 & 0.528 / 1.067\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.669 / 1.183 & 0.185 / 0.283 & 0.303 / 0.541 & 0.249 / 0.414 & 0.175 / 0.319 & 0.316 / 0.548\\
PECNet \cite{mangalam2020not} & 0.562 / 0.985 & 0.192 / 0.332 & 0.336 / 0.630 & 0.243 / 0.468 & 0.179 / 0.345 & 0.302 / 0.552\\
Y-Net no scene \cite{mangalam_goals_2020} & \textbf{0.318} / \textbf{0.377} & \underline{0.114} / \underline{0.169} & - / - & 0.213 / 0.394 & 0.147 / 0.263 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.398 / 0.571 & 0.123 / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448\\
Y-Net ped \cite{mangalam_goals_2020} & 0.404 / 0.602 & 0.154 / 0.281 & 14.144 / 27.618 & 0.254 / 0.381 & 0.174 / 0.324 & 3.026 / 5.841\\
Y-Net old \cite{mangalam_goals_2020} & \underline{0.323} / \underline{0.419} & 0.115 / \textbf{0.158} & - / - & 0.196 / 0.343 & 0.153 / 0.269 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.398 / 0.571 & 0.123 / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448\\
MemoNet \cite{Xu2022-ki} & 0.410 / 0.636 & \textbf{0.113} / 0.173 & \textbf{0.244} / \textbf{0.433} & \underline{0.184} / \underline{0.320} & 0.143 / 0.248 & \textbf{0.219} / \textbf{0.362}\\
View Vertically \cite{Wong2022-kx} & 0.569 / 0.691 & 0.124 / 0.188 & 0.290 / 0.499 & 0.202 / 0.356 & 0.147 / 0.257 & 0.267 / 0.398\\
View Vertically w/ joint loss (Ours) & 0.662 / 0.833 & 0.130 / 0.196 & 0.316 / 0.546 & 0.216 / 0.364 & 0.151 / 0.261 & 0.295 / 0.440\\
vv a 0.2-0.8 b 0.3-0.5-0.2 & 0.658 / 0.709 & - / - & - / - & - / - & - / - & - / -\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.144 / 0.221 & 0.297 / 0.522 & 0.215 / 0.390 & 0.147 / 0.257 & - / -\\
vv a 0.2,0.8 b 0.3,0.5,0.2 & 0.656 / 0.708 & 0.145 / 0.207 & 0.310 / 0.511 & 0.211 / 0.352 & 0.147 / 0.257 & 0.294 / 0.407\\
vv a 0.7,0.3 b 0.5,0.3,0.2 & 0.775 / 0.858 & 0.131 / 0.201 & 0.385 / 0.711 & 0.215 / 0.365 & 0.154 / 0.268 & 0.332 / 0.481\\
vv a 0.8,0.2 b 0.6,0.2,0.2 & 0.725 / 0.869 & 0.150 / 0.221 & 0.339 / 0.621 & 0.218 / 0.387 & 0.157 / 0.275 & 0.318 / 0.474\\
vv a 0.8,0.2 b 0.5,0.3,0.2 & 0.730 / 0.885 & 0.149 / 0.220 & 0.339 / 0.623 & 0.217 / 0.386 & 0.157 / 0.275 & 0.319 / 0.478\\
vv a 0.8,0.2 b 0.4,0.4,0.2 & 0.728 / 0.880 & 0.147 / 0.216 & 0.338 / 0.621 & 0.218 / 0.388 & 0.157 / 0.274 & 0.318 / 0.476\\
vv a 0.7,0.3 b 0.6,0.2,0.2 & 0.788 / 0.893 & 0.132 / 0.197 & 0.348 / 0.622 & 0.214 / 0.363 & 0.154 / 0.269 & 0.327 / 0.469\\
vv a 0.7,0.3 b 0.4,0.4,0.2 & 0.776 / 0.881 & 0.133 / 0.203 & 0.347 / 0.621 & 0.214 / 0.361 & 0.154 / 0.267 & 0.325 / 0.467\\
vv a 0.6,0.4 b 0.5,0.3,0.2 & 0.742 / 0.858 & 0.144 / 0.219 & 0.302 / 0.529 & 0.205 / 0.351 & 0.153 / 0.270 & 0.309 / 0.445\\
vv a 0.6,0.4 b 0.4,0.4,0.2 & 0.749 / 0.849 & 0.147 / 0.227 & 0.303 / 0.531 & 0.206 / 0.353 & 0.153 / 0.269 & 0.311 / 0.446\\
vv a 0.5,0.5 b 0.4,0.4,0.2 & 0.697 / 0.805 & 0.129 / 0.197 & 0.306 / 0.551 & 0.219 / 0.360 & \underline{0.143} / 0.246 & 0.299 / 0.432\\
vv a 0.5,0.5 b 0.5,0.3,0.2 & 0.700 / 0.792 & 0.129 / 0.196 & 0.267 / 0.474 & 0.219 / 0.359 & 0.144 / 0.247 & 0.292 / 0.414\\
vv a 0.5,0.5 b 0.6,0.2,0.2 & 0.700 / 0.800 & 0.129 / 0.199 & 0.314 / 0.579 & 0.219 / 0.355 & 0.143 / 0.246 & 0.301 / 0.436\\
AgentFormer \cite{yuan_agentformer_2021} & 0.451 / 0.748 & 0.142 / 0.225 & \underline{0.254} / \underline{0.454} & \textbf{0.177} / \textbf{0.304} & \textbf{0.140} / \textbf{0.236} & \underline{0.233} / \underline{0.393}\\
\textbf{Joint AgentFormer (Ours)} & 0.473 / 0.792 & 0.135 / 0.212 & 0.285 / 0.505 & 0.189 / 0.321 & 0.144 / \underline{0.242} & 0.245 / 0.414\\
ablation 7.5 & 0.463 / 0.729 & 0.140 / 0.222 & 0.293 / 0.523 & 0.191 / 0.330 & 0.146 / 0.249 & 0.247 / 0.411\\
\textbf{Joint AgentFormer (old)} & 0.478 / 0.774 & 0.146 / 0.236 & 0.301 / 0.543 & 0.199 / 0.349 & 0.165 / 0.293 & 0.258 / 0.439\\
ablation 10 & 0.454 / 0.743 & 0.147 / 0.239 & 0.301 / 0.544 & 0.196 / 0.340 & 0.146 / 0.250 & 0.249 / 0.423\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_max_JADE_max_JFDE}
\subfloat[\max \text{JADE}_{20} / \text{JFDE}_{20}]{
\label{table:eth_ucy_max_JADE_max_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\max \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{1.559} / \textbf{3.308} & \underline{0.930} / \underline{2.040} & \textbf{0.855} / \textbf{1.804} & \textbf{0.863} / \textbf{2.028} & \textbf{0.752} / \textbf{1.660} & \textbf{0.992} / \textbf{2.168}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 2.092 / 4.451 & 1.259 / 2.714 & 0.911 / 2.007 & \underline{1.236} / \underline{2.746} & 0.936 / \underline{2.074} & 1.287 / 2.798\\
PECNet \cite{mangalam2020not} & \underline{1.762} / \underline{3.819} & 1.048 / 2.404 & \underline{0.888} / \underline{1.932} & 1.381 / 3.208 & \underline{0.916} / 2.171 & \underline{1.199} / \underline{2.707}\\
Y-Net no scene \cite{mangalam_goals_2020} & 2.354 / 4.887 & 1.019 / 2.315 & - / - & 1.750 / 3.913 & 1.035 / 2.330 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 2.420 / 4.985 & 1.024 / 2.265 & 1.245 / 2.837 & 2.217 / 4.830 & 1.490 / 3.388 & 1.679 / 3.661\\
Y-Net ped \cite{mangalam_goals_2020} & 2.271 / 4.696 & 1.268 / 2.770 & 58.218 / 127.453 & 1.550 / 3.366 & 1.114 / 2.433 & 12.884 / 28.144\\
Y-Net old \cite{mangalam_goals_2020} & 1.861 / 3.846 & \textbf{0.923} / \textbf{1.998} & - / - & 1.461 / 3.335 & 0.949 / 2.136 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 2.420 / 4.985 & 1.024 / 2.265 & 1.245 / 2.837 & 2.217 / 4.830 & 1.490 / 3.388 & 1.679 / 3.661\\
MemoNet \cite{Xu2022-ki} & 2.650 / 5.761 & 1.816 / 3.791 & 1.055 / 2.263 & 1.403 / 3.165 & 1.277 / 3.020 & 1.640 / 3.600\\
View Vertically \cite{Wong2022-kx} & 2.770 / 5.418 & 3.701 / 6.840 & 1.496 / 2.935 & 1.859 / 4.041 & 1.348 / 2.654 & 2.235 / 4.378\\
View Vertically w/ joint loss (Ours) & 4.488 / 7.995 & 1.968 / 2.744 & 1.476 / 2.749 & 4.791 / 6.851 & 1.243 / 2.463 & 2.793 / 4.560\\
vv a 0.2-0.8 b 0.3-0.5-0.2 & 2.559 / 5.003 & - / - & - / - & - / - & - / - & - / -\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 4.008 / 5.637 & 4.406 / 6.896 & 1.826 / 3.866 & 1.295 / 2.568 & - / -\\
vv a 0.2,0.8 b 0.3,0.5,0.2 & 2.561 / 4.999 & 3.077 / 4.772 & 1.663 / 2.932 & 1.687 / 3.672 & 4.945 / 7.378 & 2.786 / 4.751\\
vv a 0.7,0.3 b 0.5,0.3,0.2 & 6.066 / 9.123 & 4.521 / 6.707 & 3.728 / 5.708 & 6.089 / 9.299 & 2.000 / 3.485 & 4.481 / 6.864\\
vv a 0.8,0.2 b 0.6,0.2,0.2 & 2.540 / 4.848 & 4.374 / 6.618 & 4.607 / 6.926 & 8.053 / 11.965 & 3.808 / 5.594 & 4.676 / 7.190\\
vv a 0.8,0.2 b 0.5,0.3,0.2 & 2.514 / 4.813 & 4.386 / 6.616 & 4.613 / 6.936 & 8.049 / 11.940 & 3.808 / 5.594 & 4.674 / 7.180\\
vv a 0.8,0.2 b 0.4,0.4,0.2 & 2.533 / 4.847 & 4.373 / 6.619 & 4.610 / 6.929 & 8.052 / 11.930 & 3.807 / 5.591 & 4.675 / 7.183\\
vv a 0.7,0.3 b 0.6,0.2,0.2 & 5.930 / 9.009 & 4.521 / 6.708 & 4.466 / 6.688 & 6.095 / 9.314 & 2.005 / 3.490 & 4.603 / 7.042\\
vv a 0.7,0.3 b 0.4,0.4,0.2 & 6.052 / 9.096 & 4.521 / 6.707 & 4.467 / 6.687 & 6.094 / 9.311 & 2.002 / 3.489 & 4.627 / 7.058\\
vv a 0.6,0.4 b 0.5,0.3,0.2 & 5.900 / 9.213 & 3.581 / 5.237 & 1.382 / 2.515 & 1.704 / 3.654 & 3.752 / 5.868 & 3.264 / 5.297\\
vv a 0.6,0.4 b 0.4,0.4,0.2 & 5.917 / 9.251 & 3.539 / 5.188 & 1.384 / 2.515 & 1.707 / 3.658 & 3.752 / 5.868 & 3.260 / 5.296\\
vv a 0.5,0.5 b 0.4,0.4,0.2 & 5.217 / 8.433 & 3.440 / 5.350 & 4.009 / 6.469 & 5.738 / 8.117 & 1.579 / 2.966 & 3.997 / 6.267\\
vv a 0.5,0.5 b 0.5,0.3,0.2 & 5.235 / 8.466 & 3.473 / 5.389 & 3.802 / 5.977 & 5.750 / 8.134 & 1.578 / 2.965 & 3.968 / 6.186\\
vv a 0.5,0.5 b 0.6,0.2,0.2 & 5.222 / 8.439 & 3.462 / 5.386 & 4.028 / 6.506 & 5.747 / 8.132 & 1.579 / 2.968 & 4.008 / 6.286\\
AgentFormer \cite{yuan_agentformer_2021} & 3.093 / 6.787 & 1.721 / 3.906 & 1.537 / 3.487 & 1.467 / 3.418 & 1.415 / 3.231 & 1.847 / 4.166\\
\textbf{Joint AgentFormer (Ours)} & 2.863 / 6.273 & 1.822 / 3.992 & 1.300 / 2.890 & 1.349 / 3.144 & 1.514 / 3.465 & 1.770 / 3.953\\
ablation 7.5 & 2.896 / 6.331 & 1.881 / 4.114 & 1.235 / 2.745 & 1.386 / 3.287 & 1.517 / 3.441 & 1.783 / 3.984\\
\textbf{Joint AgentFormer (old)} & 2.917 / 6.362 & 1.592 / 3.556 & 1.121 / 2.476 & 1.329 / 3.166 & 1.077 / 2.471 & 1.607 / 3.606\\
ablation 10 & 2.915 / 6.361 & 1.807 / 3.962 & 1.275 / 2.824 & 1.383 / 3.333 & 1.591 / 3.613 & 1.794 / 4.019\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_max_ADE_max_FDE}
\subfloat[\max \text{ADE}_{20} / \text{FDE}_{20}]{
\label{table:eth_ucy_max_ADE_max_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\max \text{ADE}_{20} / \text{FDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{1.567} / \textbf{3.372} & \textbf{1.007} / \textbf{2.218} & \textbf{0.952} / \textbf{2.000} & \textbf{0.882} / \textbf{2.055} & \textbf{0.795} / \textbf{1.781} & \textbf{1.041} / \textbf{2.285}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 2.134 / 4.597 & 1.562 / 3.375 & 1.683 / 3.716 & 1.609 / 3.553 & 1.459 / 3.201 & 1.689 / 3.688\\
PECNet \cite{mangalam2020not} & \underline{1.792} / \underline{3.944} & 1.261 / 2.875 & \underline{1.340} / \underline{2.976} & 1.789 / 4.118 & 1.301 / 3.078 & \underline{1.497} / \underline{3.398}\\
Y-Net no scene \cite{mangalam_goals_2020} & 3.086 / 6.501 & 1.388 / 3.209 & - / - & 2.337 / 5.194 & 1.542 / 3.521 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 2.733 / 5.599 & \underline{1.193} / \underline{2.647} & 1.910 / 4.326 & 2.773 / 5.979 & 2.001 / 4.550 & 2.122 / 4.620\\
Y-Net ped \cite{mangalam_goals_2020} & 2.460 / 5.094 & 1.434 / 3.131 & 84.622 / 185.765 & 1.948 / 4.265 & 1.411 / 3.074 & 18.375 / 40.266\\
Y-Net old \cite{mangalam_goals_2020} & 2.366 / 4.826 & 1.262 / 2.741 & - / - & 1.967 / 4.473 & 1.288 / 2.890 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 2.733 / 5.599 & 1.193 / 2.647 & 1.910 / 4.326 & 2.773 / 5.979 & 2.001 / 4.550 & 2.122 / 4.620\\
MemoNet \cite{Xu2022-ki} & 2.971 / 6.439 & 2.356 / 4.896 & 1.914 / 4.070 & 1.879 / 4.192 & 1.925 / 4.630 & 2.209 / 4.845\\
View Vertically \cite{Wong2022-kx} & 2.920 / 5.636 & 3.999 / 7.369 & 1.998 / 3.818 & 2.003 / 4.354 & 1.640 / 3.132 & 2.512 / 4.862\\
View Vertically w/ joint loss (Ours) & 5.041 / 9.198 & 2.061 / 2.918 & 2.024 / 3.705 & 5.325 / 7.284 & 1.360 / 2.709 & 3.162 / 5.163\\
vv a 0.2-0.8 b 0.3-0.5-0.2 & 2.673 / 5.172 & - / - & - / - & - / - & - / - & - / -\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 4.169 / 5.863 & 6.001 / 9.202 & 1.984 / 4.165 & 1.398 / 2.775 & - / -\\
vv a 0.2,0.8 b 0.3,0.5,0.2 & 2.676 / 5.173 & 3.268 / 5.063 & 2.300 / 3.963 & 1.858 / 4.016 & 5.686 / 8.411 & 3.157 / 5.326\\
vv a 0.7,0.3 b 0.5,0.3,0.2 & 6.911 / 10.327 & 4.895 / 7.267 & 5.801 / 8.652 & 6.166 / 9.704 & 2.098 / 3.628 & 5.174 / 7.915\\
vv a 0.8,0.2 b 0.6,0.2,0.2 & 2.756 / 5.216 & 4.807 / 7.194 & 5.635 / 8.472 & 9.355 / 13.935 & 3.692 / 5.496 & 5.249 / 8.063\\
vv a 0.8,0.2 b 0.5,0.3,0.2 & 2.724 / 5.168 & 4.809 / 7.177 & 5.656 / 8.502 & 9.354 / 13.924 & 3.692 / 5.497 & 5.247 / 8.054\\
vv a 0.8,0.2 b 0.4,0.4,0.2 & 2.735 / 5.183 & 4.769 / 7.150 & 5.652 / 8.492 & 9.351 / 13.931 & 3.692 / 5.495 & 5.240 / 8.050\\
vv a 0.7,0.3 b 0.6,0.2,0.2 & 6.824 / 10.276 & 4.893 / 7.264 & 6.109 / 8.945 & 6.172 / 9.715 & 2.102 / 3.633 & 5.220 / 7.967\\
vv a 0.7,0.3 b 0.4,0.4,0.2 & 6.916 / 10.313 & 4.893 / 7.263 & 6.109 / 8.944 & 6.171 / 9.714 & 2.100 / 3.631 & 5.238 / 7.973\\
vv a 0.6,0.4 b 0.5,0.3,0.2 & 6.546 / 10.143 & 4.195 / 6.085 & 2.128 / 3.608 & 1.881 / 3.987 & 4.043 / 6.430 & 3.758 / 6.051\\
vv a 0.6,0.4 b 0.4,0.4,0.2 & 6.547 / 10.141 & 4.183 / 6.088 & 2.141 / 3.623 & 1.882 / 3.991 & 4.043 / 6.431 & 3.759 / 6.055\\
vv a 0.5,0.5 b 0.4,0.4,0.2 & 5.919 / 9.486 & 3.630 / 5.639 & 5.989 / 9.293 & 5.673 / 8.182 & 1.681 / 3.129 & 4.579 / 7.145\\
vv a 0.5,0.5 b 0.5,0.3,0.2 & 5.925 / 9.500 & 3.661 / 5.681 & 5.645 / 8.530 & 5.680 / 8.195 & 1.682 / 3.131 & 4.519 / 7.007\\
vv a 0.5,0.5 b 0.6,0.2,0.2 & 5.914 / 9.480 & 3.662 / 5.689 & 6.033 / 9.327 & 5.676 / 8.185 & 1.682 / 3.132 & 4.593 / 7.163\\
AgentFormer \cite{yuan_agentformer_2021} & 3.311 / 7.274 & 1.793 / 4.051 & 1.932 / 4.396 & 1.559 / 3.614 & 1.611 / 3.675 & 2.041 / 4.602\\
\textbf{Joint AgentFormer (Ours)} & 3.007 / 6.658 & 1.856 / 4.108 & 1.642 / 3.664 & 1.347 / 3.129 & 1.639 / 3.772 & 1.898 / 4.266\\
ablation 7.5 & 3.042 / 6.723 & 1.885 / 4.147 & 1.635 / 3.643 & 1.401 / 3.304 & 1.618 / 3.717 & 1.916 / 4.307\\
\textbf{Joint AgentFormer (old)} & 3.072 / 6.774 & 1.546 / 3.495 & 1.454 / 3.247 & \underline{1.312} / \underline{3.106} & \underline{1.099} / \underline{2.552} & 1.697 / 3.835\\
ablation 10 & 3.079 / 6.787 & 1.790 / 3.964 & 1.651 / 3.680 & 1.401 / 3.354 & 1.726 / 3.944 & 1.930 / 4.346\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}

==> tables/baseline.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{Baseline evaluations across SOTA baselines (first 7 rows) as well as Our method (last row), on the ETH / UCY datasets (first 6 columns) and the Stanford Drone dataset (last column). The metric benig reported (a. \textit{SADE} / \textit{SFDE}, b. $CR_{SADE}$ / $CR_{mean}$, and c. \textit{ADE} / \textit{FDE}) is shown in the title of each table. Sequence density, as given by mean number of agents per 20-frame sequence, is shown in parentheses next to each dataset name. Lower is better; bolded values show best result, underlined shows second-best. All results are for $K=20$ prediction samples per sequence.}

\label{table:all_results}
\subfloat[\textit{SADE} / \textit{SFDE}]{
\label{table:eth_ucy_min_SADE_min_SFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min SADE_{20} / \text{SFDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg. & SDD TrajNet \footnotesize(1.5)\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.919 / 1.742 & 0.480 / 0.950 & 0.744 / 1.573 & 0.438 / 1.001 & 0.362 / 0.794 & 0.589 / 1.212 & 13.764 / 24.843\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.726 / 1.299 & 0.237 / 0.418 & \underline{0.609} / 1.316 & 0.359 / 0.712 & \underline{0.294} / 0.625 & 0.445 / 0.874 & 11.359 / 18.208\\
PECNet \cite{mangalam2020not} & 0.618 / 1.097 & 0.291 / 0.587 & 0.666 / 1.417 & 0.408 / 0.896 & 0.372 / 0.840 & 0.471 / 0.967 & 10.824 / 19.478\\
Y-Net \cite{mangalam_goals_2020} & 0.495 / 0.781 & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974 & 9.671 / \textbf{16.010}\\
MemoNet \cite{Xu2022-ki} & 0.499 / 0.859 & 0.222 / 0.416 & 0.686 / 1.466 & 0.349 / 0.723 & 0.385 / 0.864 & 0.428 / 0.866 & \underline{9.590} / 16.430\\
View Vertically \cite{Wong2022-kx} & 0.561 / \textbf{0.776} & \underline{0.196} / \textbf{0.332} & 0.654 / \underline{1.307} & 0.328 / 0.654 & 0.298 / \underline{0.602} & 0.408 / \underline{0.734} & 10.747 / 17.447\\
AgentFormer \cite{yuan_agentformer_2021} & \textbf{0.482} / 0.794 & 0.237 / 0.456 & 0.622 / 1.310 & \underline{0.285} / \underline{0.564} & 0.296 / 0.624 & \underline{0.384} / 0.749 & 9.673 / 16.920\\
\textbf{Joint AgentFormer (Ours)} & \underline{0.486} / \underline{0.780} & \textbf{0.194} / \underline{0.338} & \textbf{0.602} / \textbf{1.246} & \textbf{0.267} / \textbf{0.513} & \textbf{0.242} / \textbf{0.482} & \textbf{0.358} / \textbf{0.672} & \textbf{9.417} / \underline{16.207}\\
\hline
\end{tabular}
} % resize box
} % subfloat




\subfloat[$CR_{SADE}$ / $CR_{mean}$]{
\label{table:eth_ucy_mean_collision_rate_max_collision_rate}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{CR_{mean} / \text{CR}_{SADE} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg. & SDD TrajNet \footnotesize(1.5)\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.015 / \textbf{0.045} & 0.031 / 0.090 & \underline{0.165} / \textbf{0.251} & 0.060 / 0.185 & 0.083 / 0.195 & 0.071 / \underline{0.153} & 0.000 / 0.002\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.025 / 0.137 & 0.044 / 0.271 & 0.281 / 0.489 & 0.088 / 0.466 & 0.126 / 0.456 & 0.113 / 0.364 & 0.000 / 0.004\\
PECNet \cite{mangalam2020not} & \underline{0.014} / 0.115 & 0.043 / 0.269 & 0.218 / 0.409 & 0.059 / 0.396 & 0.128 / 0.455 & 0.092 / 0.329 & 0.005 / 0.033\\
Y-Net \cite{mangalam_goals_2020} & 0.016 / 0.141 & 0.039 / 0.250 & 0.265 / 0.482 & 0.100 / 0.513 & 0.134 / 0.480 & 0.111 / 0.373 & 0.000 / 0.002\\
MemoNet \cite{Xu2022-ki} & 0.014 / 0.160 & 0.040 / 0.301 & 0.206 / 0.415 & 0.065 / 0.445 & 0.136 / 0.483 & 0.092 / 0.361 & 0.000 / 0.004\\
View Vertically \cite{Wong2022-kx} & 0.014 / 0.090 & 0.029 / 0.203 & 0.212 / 0.428 & 0.045 / 0.233 & 0.082 / 0.316 & 0.077 / 0.254 & 0.000 / 0.003\\
AgentFormer \cite{yuan_agentformer_2021} & 0.016 / \underline{0.068} & \underline{0.022} / \underline{0.084} & 0.204 / 0.362 & \underline{0.021} / \textbf{0.088} & \underline{0.054} / \textbf{0.139} & \underline{0.063} / \textbf{0.148} & \textbf{0.000} / \textbf{0.000}\\
\textbf{Joint AgentFormer (Ours)} & \textbf{0.012} / 0.069 & \textbf{0.016} / \textbf{0.069} & \textbf{0.163} / \underline{0.338} & \textbf{0.020} / \underline{0.099} & \textbf{0.054} / \underline{0.195} & \textbf{0.053} / 0.154 & \underline{0.000} / \underline{0.000}\\
\hline
Ground Truth & 0.000 & 0.001 & 0.021 & 0.000 & 0.002 & 0.005 & 0.000\\
\hline
\end{tabular}
} % resize box
} % subfloat



\subfloat[\textit{ADE} / \textit{FDE}]{
\label{table:eth_ucy_min_ADE_min_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min ADE_{20} / \text{FDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg. & SDD TrajNet \footnotesize(1.5)\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.876 / 1.656 & 0.461 / 0.920 & 0.639 / 1.343 & 0.379 / 0.816 & 0.285 / 0.600 & 0.528 / 1.067 & 12.740 / 22.654\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.669 / 1.183 & 0.185 / 0.283 & 0.303 / 0.541 & 0.249 / 0.414 & 0.175 / 0.319 & 0.316 / 0.548 & 10.181 / 15.756\\
PECNet \cite{mangalam2020not} & 0.562 / 0.985 & 0.192 / 0.332 & 0.336 / 0.630 & 0.243 / 0.468 & 0.179 / 0.345 & 0.302 / 0.552 & 9.343 / 16.104\\
Y-Net \cite{mangalam_goals_2020} & \textbf{0.398} / \textbf{0.571} & \underline{0.123} / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448 & 8.151 / \textbf{12.803}\\
MemoNet \cite{Xu2022-ki} & \underline{0.410} / \underline{0.636} & \textbf{0.113} / \textbf{0.173} & \textbf{0.244} / \textbf{0.433} & \underline{0.184} / \underline{0.320} & \underline{0.143} / \underline{0.248} & \textbf{0.219} / \textbf{0.362} & \textbf{7.966} / \underline{12.822}\\
View Vertically \cite{Wong2022-kx} & 0.569 / 0.691 & 0.124 / \underline{0.188} & 0.290 / 0.499 & 0.202 / 0.356 & 0.147 / 0.257 & 0.267 / 0.398 & 9.337 / 14.666\\
AgentFormer \cite{yuan_agentformer_2021} & 0.451 / 0.748 & 0.142 / 0.225 & \underline{0.254} / \underline{0.454} & \textbf{0.177} / \textbf{0.304} & \textbf{0.140} / \textbf{0.236} & \underline{0.233} / \underline{0.393} & \underline{8.005} / 13.243\\
\textbf{Joint AgentFormer (Ours)} & 0.478 / 0.774 & 0.146 / 0.236 & 0.301 / 0.543 & 0.199 / 0.349 & 0.165 / 0.293 & 0.258 / 0.439 & 8.211 / 13.698\\
\hline
\end{tabular}
} % resize
} % subfload
\end{table*}



==> tables/baseline_int_cats.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{Baseline comparison (\textit{JADE} / \textit{JFDE}) on interaction category cross-sections (leader-follower, group, collision-avoidance).}
\label{table:baseline_int_cats}
\subfloat[leader-follower]{
\label{table:eth_ucy_min_JADE_min_JFDE_leader-follower}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min JADE_{20} / \text{JFDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 2.008 / 4.322 & 0.540 / 0.976 & 0.590 / 1.242 & 0.489 / 1.059 & 0.280 / 0.535 & 0.781 / 1.627 & 8.535 / 16.562\\
Trajectron++ \cite{salzmann_trajectron_2021} & 1.016 / 2.157 & 0.421 / 0.764 & 0.368 / 0.723 & 0.342 / 0.592 & 0.363 / 0.715 & 0.502 / 0.990 & 9.535 / 15.782\\
PECNet \cite{mangalam2020not} & 1.018 / 2.286 & 0.468 / 0.826 & 0.421 / 0.846 & 0.339 / 0.706 & 0.373 / 0.767 & 0.524 / 1.086 & \textbf{6.939} / \textbf{10.530}\\
Y-Net \cite{mangalam_goals_2020} & \textbf{0.874} / \underline{1.918} & 0.444 / 0.852 & 0.479 / 1.039 & 0.389 / 0.781 & 0.630 / 1.381 & 0.563 / 1.194 & 9.312 / 17.636\\
MemoNet \cite{Xu2022-ki} & \underline{0.949} / 2.050 & 0.319 / 0.637 & \underline{0.350} / 0.705 & 0.298 / 0.591 & 0.327 / 0.632 & \textbf{0.449} / \underline{0.923} & 8.366 / 15.745\\
View Vertically \cite{Wong2022-kx} & 1.519 / \textbf{1.176} & 0.290 / 0.474 & 0.358 / \textbf{0.664} & 0.378 / 0.710 & 0.307 / 0.564 & 0.571 / \textbf{0.718} & 8.066 / 16.782\\
AgentFormer \cite{yuan_agentformer_2021} & 1.113 / 2.726 & \underline{0.285} / \underline{0.466} & 0.355 / 0.708 & \underline{0.261} / \underline{0.481} & \underline{0.257} / \underline{0.462} & \underline{0.454} / 0.969 & \underline{7.800} / \underline{13.139}\\
\textbf{Joint AgentFormer (Ours)} & 1.257 / 2.646 & \textbf{0.265} / \textbf{0.434} & \textbf{0.346} / \underline{0.666} & \textbf{0.250} / \textbf{0.456} & \textbf{0.244} / \textbf{0.422} & 0.472 / 0.925 & 8.530 / 16.140\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_JADE_min_JFDE_group}
\subfloat[group]{
\label{table:eth_ucy_min_JADE_min_JFDE_group}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min JADE_{20} / \text{JFDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.802 / 1.608 & 0.548 / 1.111 & 0.698 / 1.469 & 0.412 / 0.902 & 0.282 / 0.592 & 0.548 / 1.137 & 7.715 / 13.743\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.665 / 1.348 & 0.289 / 0.527 & \underline{0.541} / 1.156 & 0.374 / 0.762 & 0.246 / 0.516 & 0.423 / 0.862 & 8.173 / 14.799\\
PECNet \cite{mangalam2020not} & 0.589 / 1.236 & 0.357 / 0.731 & 0.598 / 1.265 & 0.437 / 0.963 & 0.331 / 0.754 & 0.462 / 0.990 & 8.484 / 17.926\\
Y-Net \cite{mangalam_goals_2020} & 0.680 / 1.248 & 0.282 / 0.556 & 0.643 / 1.449 & 0.518 / 1.131 & 0.455 / 1.025 & 0.515 / 1.082 & 8.913 / 16.766\\
MemoNet \cite{Xu2022-ki} & 0.619 / 1.309 & 0.275 / 0.523 & 0.589 / 1.251 & 0.356 / 0.753 & 0.336 / 0.766 & 0.435 / 0.920 & 8.049 / 15.509\\
View Vertically \cite{Wong2022-kx} & 0.681 / \textbf{0.721} & \underline{0.229} / \underline{0.406} & 0.551 / \underline{1.089} & 0.307 / 0.603 & 0.228 / 0.443 & 0.399 / \underline{0.652} & 7.276 / 12.564\\
AgentFormer \cite{yuan_agentformer_2021} & \textbf{0.468} / \underline{0.904} & 0.248 / 0.463 & 0.560 / 1.176 & \underline{0.257} / \underline{0.486} & \underline{0.208} / \underline{0.411} & \underline{0.348} / 0.688 & \textbf{6.122} / \textbf{10.739}\\
\textbf{Joint AgentFormer (Ours)} & \underline{0.548} / 1.021 & \textbf{0.195} / \textbf{0.319} & \textbf{0.523} / \textbf{1.071} & \textbf{0.248} / \textbf{0.462} & \textbf{0.181} / \textbf{0.338} & \textbf{0.339} / \textbf{0.642} & \underline{6.660} / \underline{11.808}\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_JADE_min_JFDE_collision_avoidance}
\subfloat[collision avoidance]{
\label{table:eth_ucy_min_JADE_min_JFDE_collision_avoidance}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min JADE_{20} / \text{JFDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 1.305 / 2.475 & 0.567 / 1.086 & 0.789 / 1.682 & 0.413 / 0.826 & 0.511 / 1.076 & 0.717 / 1.429 & 17.702 / 37.887\\
Trajectron++ \cite{salzmann_trajectron_2021} & 1.662 / 3.797 & 0.299 / 0.535 & 0.668 / 1.439 & 0.411 / 0.829 & 0.490 / 1.027 & 0.706 / 1.526 & 17.258 / 34.967\\
PECNet \cite{mangalam2020not} & 1.600 / 3.537 & 0.343 / 0.641 & 0.688 / 1.447 & 0.460 / 0.981 & 0.461 / 0.967 & 0.710 / 1.515 & 14.591 / 32.196\\
Y-Net \cite{mangalam_goals_2020} & \underline{0.917} / \underline{1.234} & 0.214 / \underline{0.320} & 0.746 / 1.675 & 0.508 / 1.082 & 0.661 / 1.459 & 0.609 / 1.154 & 17.384 / 37.339\\
MemoNet \cite{Xu2022-ki} & 1.035 / 1.867 & 0.235 / 0.377 & 0.699 / 1.485 & 0.389 / 0.770 & 0.475 / 0.973 & 0.567 / 1.094 & 13.238 / 27.051\\
View Vertically \cite{Wong2022-kx} & 1.267 / 1.417 & \textbf{0.199} / 0.351 & 0.693 / 1.375 & 0.388 / 0.771 & 0.479 / 0.977 & 0.605 / 0.978 & 15.640 / 31.846\\
AgentFormer \cite{yuan_agentformer_2021} & \textbf{0.743} / \textbf{1.113} & 0.318 / 0.603 & \underline{0.647} / \underline{1.368} & \underline{0.342} / \underline{0.671} & \underline{0.424} / \underline{0.860} & \textbf{0.495} / \underline{0.923} & \underline{13.233} / \textbf{24.591}\\
\textbf{Joint AgentFormer (Ours)} & 0.994 / 1.624 & \underline{0.207} / \textbf{0.278} & \textbf{0.634} / \textbf{1.317} & \textbf{0.309} / \textbf{0.579} & \textbf{0.407} / \textbf{0.816} & \underline{0.510} / \textbf{0.923} & \textbf{12.876} / \underline{26.706}\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{Baseline comparison ($CR_{JADE}$ / $CR_{mean}$) on interaction category cross-sections (leader-follower, group, collision-avoidance).}
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_leader-follower}
\subfloat[leader-follower]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_leader-follower}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{CR_{JADE} / \text{CR}_{mean} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{0.000} / \textbf{0.000} & \textbf{0.000} / \textbf{0.014} & \textbf{0.244} / \underline{0.260} & 0.143 / 0.138 & 0.140 / 0.146 & \textbf{0.105} / \underline{0.112} & \textbf{0.000} / \textbf{0.000}\\
Trajectron++ \cite{salzmann_trajectron_2021} & \underline{0.000} / 0.025 & 0.091 / 0.109 & 0.474 / 0.462 & 0.143 / 0.188 & 0.218 / 0.230 & 0.185 / 0.203 & \underline{0.000} / 0.006\\
PECNet \cite{mangalam2020not} & 0.000 / \underline{0.000} & \underline{0.000} / 0.050 & 0.315 / 0.335 & \textbf{0.100} / 0.155 & \underline{0.134} / 0.172 & 0.110 / 0.142 & 0.125 / 0.025\\
Y-Net \cite{mangalam_goals_2020} & 0.000 / 0.050 & 0.000 / 0.109 & 0.343 / 0.414 & \underline{0.100} / 0.164 & 0.190 / 0.194 & 0.127 / 0.186 & 0.000 / \underline{0.000}\\
MemoNet \cite{Xu2022-ki} & 0.000 / 0.000 & 0.000 / 0.086 & 0.279 / 0.297 & 0.114 / 0.146 & 0.151 / 0.188 & \underline{0.109} / 0.143 & 0.000 / 0.013\\
View Vertically \cite{Wong2022-kx} & 0.000 / 0.013 & 0.000 / 0.055 & 0.348 / 0.350 & 0.114 / 0.099 & \textbf{0.123} / \textbf{0.132} & 0.117 / 0.130 & 0.000 / 0.000\\
AgentFormer \cite{yuan_agentformer_2021} & 0.000 / 0.025 & 0.000 / \underline{0.032} & 0.321 / 0.332 & 0.129 / \underline{0.076} & 0.156 / 0.154 & 0.121 / 0.124 & 0.000 / 0.000\\
\textbf{Joint AgentFormer (Ours)} & 0.000 / 0.000 & 0.000 / 0.055 & \underline{0.255} / \textbf{0.257} & 0.143 / \textbf{0.051} & 0.162 / \underline{0.138} & 0.112 / \textbf{0.100} & 0.000 / 0.000\\
\hline
Ground Truth & 0.000 & 0.000 & 0.142 & 0.000 & 0.000 & 0.028 & 0.000\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_group}
\subfloat[group]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_group}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{CR_{JADE} / \text{CR}_{mean} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{0.029} / \textbf{0.035} & 0.060 / 0.067 & \underline{0.203} / \underline{0.201} & 0.092 / 0.099 & 0.106 / 0.121 & 0.098 / 0.105 & \textbf{0.000} / 0.003\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.221 / 0.186 & 0.101 / 0.112 & 0.355 / 0.376 & 0.169 / 0.171 & 0.149 / 0.190 & 0.199 / 0.207 & \underline{0.000} / 0.003\\
PECNet \cite{mangalam2020not} & \underline{0.074} / 0.104 & 0.101 / 0.110 & 0.287 / 0.292 & 0.102 / 0.121 & 0.171 / 0.191 & 0.147 / 0.163 & 0.086 / 0.065\\
Y-Net \cite{mangalam_goals_2020} & 0.221 / 0.118 & 0.077 / 0.102 & 0.276 / 0.350 & 0.138 / 0.193 & 0.147 / 0.200 & 0.172 / 0.192 & 0.000 / \textbf{0.000}\\
MemoNet \cite{Xu2022-ki} & 0.221 / \underline{0.082} & 0.054 / 0.093 & 0.258 / 0.277 & 0.133 / 0.126 & 0.188 / 0.203 & 0.171 / 0.156 & 0.000 / 0.003\\
View Vertically \cite{Wong2022-kx} & 0.118 / 0.107 & 0.060 / 0.073 & 0.231 / 0.267 & 0.075 / 0.093 & 0.082 / 0.102 & 0.113 / 0.128 & 0.000 / 0.001\\
AgentFormer \cite{yuan_agentformer_2021} & 0.074 / 0.088 & \underline{0.048} / \underline{0.049} & 0.228 / 0.254 & \underline{0.038} / \underline{0.045} & \underline{0.075} / \textbf{0.079} & \underline{0.093} / \underline{0.103} & 0.000 / \underline{0.000}\\
\textbf{Joint AgentFormer (Ours)} & 0.074 / 0.089 & \textbf{0.014} / \textbf{0.038} & \textbf{0.187} / \textbf{0.196} & \textbf{0.032} / \textbf{0.035} & \textbf{0.066} / \underline{0.080} & \textbf{0.074} / \textbf{0.087} & 0.000 / 0.000\\
\hline
Ground Truth & 0.000 & 0.004 & 0.040 & 0.000 & 0.005 & 0.010 & 0.000\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_collision_avoidance}
\subfloat[collision avoidance]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate_collision_avoidance}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{CR_{JADE} / \text{CR}_{mean} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \underline{0.087} / 0.100 & 0.102 / \underline{0.107} & 0.273 / 0.270 & \textbf{0.125} / \textbf{0.137} & 0.258 / 0.259 & 0.169 / \underline{0.175} & \textbf{0.000} / \textbf{0.000}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.174 / 0.139 & 0.184 / 0.138 & 0.405 / 0.421 & 0.201 / 0.252 & 0.236 / 0.257 & 0.240 / 0.241 & \underline{0.000} / 0.004\\
PECNet \cite{mangalam2020not} & 0.087 / \underline{0.098} & 0.102 / 0.139 & 0.321 / 0.319 & 0.178 / 0.217 & 0.246 / 0.245 & 0.187 / 0.204 & 0.000 / 0.005\\
Y-Net \cite{mangalam_goals_2020} & 0.174 / 0.165 & 0.102 / 0.124 & 0.321 / 0.374 & 0.254 / 0.257 & \underline{0.218} / 0.256 & 0.214 / 0.236 & 0.000 / 0.004\\
MemoNet \cite{Xu2022-ki} & \textbf{0.043} / \textbf{0.050} & \textbf{0.020} / \textbf{0.066} & \textbf{0.246} / \textbf{0.259} & 0.250 / 0.218 & 0.244 / 0.249 & \underline{0.161} / \textbf{0.169} & 0.000 / \underline{0.000}\\
View Vertically \cite{Wong2022-kx} & 0.261 / 0.137 & 0.184 / 0.167 & 0.304 / 0.326 & 0.186 / 0.198 & 0.232 / 0.215 & 0.233 / 0.209 & 0.000 / 0.004\\
AgentFormer \cite{yuan_agentformer_2021} & 0.217 / 0.178 & 0.102 / 0.108 & 0.313 / 0.329 & 0.133 / 0.185 & 0.221 / \textbf{0.207} & 0.197 / 0.201 & 0.000 / 0.000\\
\textbf{Joint AgentFormer (Ours)} & 0.130 / 0.161 & \underline{0.082} / 0.142 & \underline{0.271} / \underline{0.269} & \underline{0.125} / \underline{0.166} & \textbf{0.187} / \underline{0.211} & \textbf{0.159} / 0.190 & 0.000 / 0.002\\
\hline
Ground Truth & 0.000 & 0.000 & 0.042 & 0.000 & 0.014 & 0.011 & 0.071\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{Baseline comparison (\ADE / \FDE) on interaction category cross-sections (leader-follower, group, collision-avoidance).}
\label{table:eth_ucy_min_ADE_min_FDE_leader-follower}
\subfloat[leader-follower]{
\label{table:eth_ucy_min_ADE_min_FDE_leader-follower}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min ADE_{20} / \text{FDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 2.007 / 4.322 & 0.526 / 0.945 & 0.554 / 1.165 & 0.421 / 0.865 & 0.242 / 0.446 & 0.750 / 1.549 & 7.814 / 12.891\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.891 / 1.940 & 0.299 / 0.589 & 0.259 / 0.422 & 0.249 / 0.330 & 0.223 / 0.364 & 0.384 / 0.729 & 8.027 / 12.175\\
PECNet \cite{mangalam2020not} & 0.926 / 2.015 & 0.317 / 0.444 & 0.279 / 0.504 & 0.204 / 0.385 & 0.240 / 0.413 & 0.393 / 0.752 & \underline{5.189} / \underline{7.520}\\
Y-Net \cite{mangalam_goals_2020} & \underline{0.487} / 1.114 & 0.262 / 0.396 & 0.278 / 0.531 & 0.226 / 0.423 & 0.291 / 0.605 & \underline{0.309} / 0.614 & 6.278 / 11.328\\
MemoNet \cite{Xu2022-ki} & \textbf{0.486} / \underline{0.985} & 0.216 / 0.349 & \textbf{0.193} / \textbf{0.337} & \underline{0.174} / 0.288 & \textbf{0.180} / 0.281 & \textbf{0.250} / \underline{0.448} & \textbf{4.172} / \textbf{5.215}\\
View Vertically \cite{Wong2022-kx} & 1.471 / \textbf{0.800} & \textbf{0.207} / \underline{0.337} & 0.243 / \underline{0.401} & 0.203 / 0.328 & 0.190 / 0.294 & 0.463 / \textbf{0.432} & 5.268 / 10.524\\
AgentFormer \cite{yuan_agentformer_2021} & 1.081 / 2.645 & 0.224 / 0.373 & \underline{0.235} / 0.444 & \textbf{0.167} / \textbf{0.246} & \underline{0.181} / \underline{0.274} & 0.378 / 0.796 & 6.594 / 11.767\\
\textbf{Joint AgentFormer (Ours)} & 1.215 / 2.645 & \underline{0.212} / \textbf{0.276} & 0.257 / 0.453 & 0.183 / \underline{0.278} & 0.184 / \textbf{0.265} & 0.410 / 0.783 & 5.562 / 10.326\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_ADE_min_FDE_group}
\subfloat[group]{
\label{table:eth_ucy_min_ADE_min_FDE_group}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min ADE_{20} / \text{FDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.766 / 1.520 & 0.508 / 1.021 & 0.618 / 1.299 & 0.364 / 0.784 & 0.238 / 0.486 & 0.499 / 1.022 & 5.921 / 9.849\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.537 / 0.964 & 0.196 / 0.299 & 0.284 / 0.489 & 0.234 / 0.378 & 0.149 / 0.264 & 0.280 / 0.479 & 6.149 / 8.850\\
PECNet \cite{mangalam2020not} & 0.451 / 0.893 & 0.212 / 0.371 & 0.313 / 0.583 & 0.231 / 0.443 & 0.151 / 0.295 & 0.272 / 0.517 & 5.480 / 9.351\\
Y-Net \cite{mangalam_goals_2020} & \underline{0.372} / \textbf{0.545} & 0.143 / 0.230 & 0.296 / 0.573 & 0.250 / 0.476 & 0.182 / 0.364 & 0.248 / 0.438 & 5.422 / 9.207\\
MemoNet \cite{Xu2022-ki} & \textbf{0.350} / 0.603 & \textbf{0.122} / \textbf{0.194} & \textbf{0.222} / \textbf{0.388} & \underline{0.170} / 0.298 & \underline{0.119} / 0.204 & \textbf{0.197} / \textbf{0.337} & \textbf{4.892} / \textbf{7.995}\\
View Vertically \cite{Wong2022-kx} & 0.650 / \underline{0.589} & \underline{0.131} / \underline{0.206} & 0.267 / 0.453 & 0.188 / 0.327 & 0.121 / 0.209 & 0.271 / \underline{0.357} & 5.503 / 8.940\\
AgentFormer \cite{yuan_agentformer_2021} & 0.452 / 0.870 & 0.159 / 0.251 & \underline{0.246} / \underline{0.447} & \textbf{0.165} / \textbf{0.282} & \textbf{0.116} / \textbf{0.187} & \underline{0.228} / 0.408 & \underline{5.272} / \underline{8.825}\\
\textbf{Joint AgentFormer (Ours)} & 0.526 / 0.997 & 0.145 / 0.228 & 0.275 / 0.495 & 0.171 / \underline{0.290} & 0.119 / \underline{0.193} & 0.247 / 0.440 & 5.482 / 9.604\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_ADE_min_FDE_collision_avoidance}
\subfloat[collision avoidance]{
\label{table:eth_ucy_min_ADE_min_FDE_collision_avoidance}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c||c}
\hline
\noalign{\smallskip}
 & \multicolumn{7}{c}{min ADE_{20} / \text{FDE}_{20} $\downarrow$  (m),  $K=20$ samples} \\
\cline{2-8}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & ETH / UCY Avg. & TrajNet SDD\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 1.254 / 2.376 & 0.521 / 0.998 & 0.698 / 1.483 & 0.354 / 0.679 & 0.449 / 0.929 & 0.655 / 1.293 & 14.344 / 30.195\\
Trajectron++ \cite{salzmann_trajectron_2021} & 1.557 / 3.413 & 0.260 / 0.430 & 0.362 / 0.647 & 0.280 / 0.464 & 0.351 / 0.659 & 0.562 / 1.123 & 14.955 / 26.712\\
PECNet \cite{mangalam2020not} & 1.468 / 3.180 & 0.265 / 0.422 & 0.378 / 0.703 & 0.277 / 0.510 & 0.324 / 0.598 & 0.542 / 1.083 & \textbf{9.937} / 19.707\\
Y-Net \cite{mangalam_goals_2020} & \textbf{0.595} / \textbf{0.650} & \underline{0.156} / \underline{0.194} & 0.372 / 0.724 & 0.262 / 0.471 & 0.345 / 0.669 & 0.346 / 0.542 & 12.781 / 24.897\\
MemoNet \cite{Xu2022-ki} & 0.794 / 1.171 & \textbf{0.154} / 0.217 & \underline{0.286} / \textbf{0.505} & 0.200 / 0.345 & 0.270 / 0.456 & \underline{0.341} / \underline{0.538} & \underline{10.090} / \underline{18.841}\\
View Vertically \cite{Wong2022-kx} & 1.189 / 1.265 & 0.166 / 0.226 & 0.346 / 0.591 & 0.223 / 0.391 & 0.293 / 0.509 & 0.444 / 0.596 & 12.899 / 24.043\\
AgentFormer \cite{yuan_agentformer_2021} & \underline{0.720} / \underline{1.098} & 0.176 / 0.211 & \textbf{0.284} / \underline{0.509} & \textbf{0.177} / \textbf{0.273} & \textbf{0.260} / \textbf{0.436} & \textbf{0.324} / \textbf{0.505} & 10.456 / \textbf{17.952}\\
\textbf{Joint AgentFormer (Ours)} & 0.925 / 1.593 & 0.166 / \textbf{0.193} & 0.319 / 0.565 & \underline{0.189} / \underline{0.302} & \underline{0.269} / \underline{0.452} & 0.374 / 0.621 & 10.369 / 19.643\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}

==> tables/int_cats.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{}
\label{table:eth_ucy_min_JADE_min_JFDE}
\subfloat[\textit{JADE} / \textit{JFDE}]{
\label{table:eth_ucy_min_JADE_min_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.919 / 1.742 & 0.480 / 0.950 & 0.744 / 1.573 & 0.438 / 1.001 & 0.362 / 0.794 & 0.589 / 1.212\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.726 / 1.299 & 0.237 / 0.418 & 0.609 / 1.316 & 0.359 / 0.712 & 0.294 / 0.625 & 0.445 / 0.874\\
PECNet \cite{mangalam2020not} & 0.618 / 1.097 & 0.291 / 0.587 & 0.666 / 1.417 & 0.408 / 0.896 & 0.372 / 0.840 & 0.471 / 0.967\\
Y-Net no scene \cite{mangalam_goals_2020} & 0.479 / 0.785 & 0.215 / 0.423 & - / - & 0.401 / 0.867 & 0.318 / 0.680 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.495 / 0.781 & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974\\
Y-Net ped \cite{mangalam_goals_2020} & 0.486 / 0.784 & 0.293 / 0.610 & 33.918 / 73.481 & 0.407 / 0.718 & 0.332 / 0.704 & 7.087 / 15.260\\
Y-Net old \cite{mangalam_goals_2020} & 0.489 / 0.868 & 0.230 / 0.413 & - / - & 0.377 / 0.785 & 0.336 / 0.717 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.495 / 0.781 & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974\\
MemoNet \cite{Xu2022-ki} & 0.499 / 0.859 & 0.222 / 0.416 & 0.686 / 1.466 & 0.349 / 0.723 & 0.385 / 0.864 & 0.428 / 0.866\\
View Vertically \cite{Wong2022-kx} & 0.561 / 0.776 & 0.196 / 0.332 & 0.654 / 1.307 & 0.328 / 0.654 & 0.298 / 0.602 & 0.408 / 0.734\\
View Vertically w/ joint loss (Ours) & 0.651 / 0.924 & \textbf{0.182} / \textbf{0.303} & 0.628 / 1.263 & 0.334 / 0.645 & 0.269 / 0.544 & 0.413 / 0.736\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.202 / 0.326 & 0.602 / \underline{1.233} & 0.332 / 0.657 & 0.263 / 0.529 & - / -\\
AgentFormer \cite{yuan_agentformer_2021} & 0.482 / 0.794 & 0.237 / 0.456 & 0.622 / 1.310 & 0.285 / 0.564 & 0.296 / 0.624 & 0.384 / 0.749\\
\textbf{Joint AgentFormer (Ours)} & 0.485 / 0.798 & \underline{0.186} / \underline{0.320} & \textbf{0.590} / \textbf{1.219} & \underline{0.271} / \underline{0.513} & 0.252 / 0.509 & \textbf{0.357} / \textbf{0.672}\\
ablation 7.5 & \underline{0.477} / \textbf{0.747} & 0.191 / 0.335 & 0.609 / 1.262 & 0.272 / 0.524 & \underline{0.248} / \underline{0.502} & 0.360 / 0.674\\
\textbf{Joint AgentFormer (old)} & 0.486 / 0.780 & 0.194 / 0.338 & \underline{0.602} / 1.246 & \textbf{0.267} / \textbf{0.513} & \textbf{0.242} / \textbf{0.482} & \underline{0.358} / \underline{0.672}\\
ablation 10 & \textbf{0.465} / \underline{0.755} & 0.193 / 0.334 & 0.608 / 1.256 & 0.273 / 0.529 & 0.260 / 0.525 & 0.360 / 0.680\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\subfloat[$CR_{JADE}$ / $CR_{mean}$]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\text{CR}_{JADE} / \text{CR}_{mean} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.021 / 0.015 & 0.025 / 0.031 & 0.165 / 0.165 & 0.057 / 0.060 & 0.074 / 0.083 & 0.068 / 0.071\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.031 / 0.025 & 0.038 / 0.044 & 0.267 / 0.281 & 0.083 / 0.088 & 0.092 / 0.126 & 0.102 / 0.113\\
PECNet \cite{mangalam2020not} & \textbf{0.009} / 0.014 & 0.037 / 0.043 & 0.211 / 0.218 & 0.050 / 0.059 & 0.112 / 0.128 & 0.084 / 0.092\\
Y-Net no scene \cite{mangalam_goals_2020} & 0.044 / 0.062 & 0.023 / 0.075 & - / - & 0.051 / 0.114 & 0.073 / 0.141 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.028 / 0.016 & 0.030 / 0.039 & 0.209 / 0.265 & 0.065 / 0.100 & 0.097 / 0.134 & 0.086 / 0.111\\
Y-Net ped \cite{mangalam_goals_2020} & 0.019 / 0.016 & 0.042 / 0.044 & \textbf{0.005} / \textbf{0.007} & 0.039 / 0.068 & 0.072 / 0.098 & \textbf{0.035} / \textbf{0.047}\\
Y-Net old \cite{mangalam_goals_2020} & 0.071 / 0.062 & 0.035 / 0.073 & - / - & 0.058 / 0.104 & 0.087 / 0.120 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.028 / 0.016 & 0.030 / 0.039 & 0.209 / 0.265 & 0.065 / 0.100 & 0.097 / 0.134 & 0.086 / 0.111\\
MemoNet \cite{Xu2022-ki} & 0.031 / 0.014 & 0.034 / 0.040 & 0.192 / 0.206 & 0.060 / 0.065 & 0.119 / 0.136 & 0.087 / 0.092\\
View Vertically \cite{Wong2022-kx} & 0.012 / 0.014 & 0.020 / 0.029 & 0.187 / 0.212 & 0.034 / 0.045 & 0.059 / 0.082 & 0.062 / 0.077\\
View Vertically w/ joint loss (Ours) & 0.023 / 0.015 & 0.024 / 0.032 & 0.187 / 0.216 & 0.030 / 0.050 & 0.058 / 0.075 & 0.064 / 0.077\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.021 / 0.035 & 0.174 / 0.213 & 0.032 / 0.043 & 0.053 / 0.077 & - / -\\
AgentFormer \cite{yuan_agentformer_2021} & \underline{0.012} / 0.016 & 0.019 / 0.022 & 0.182 / 0.204 & \underline{0.014} / 0.021 & 0.048 / \underline{0.054} & 0.055 / 0.063\\
\textbf{Joint AgentFormer (Ours)} & 0.017 / 0.013 & 0.011 / 0.019 & 0.159 / 0.163 & 0.015 / 0.021 & \underline{0.041} / 0.055 & 0.049 / 0.054\\
ablation 7.5 & 0.015 / \underline{0.012} & \textbf{0.006} / 0.019 & \underline{0.149} / \underline{0.154} & \textbf{0.012} / \textbf{0.020} & 0.044 / 0.056 & \underline{0.045} / \underline{0.052}\\
\textbf{Joint AgentFormer (old)} & 0.013 / \textbf{0.012} & 0.010 / \textbf{0.016} & 0.150 / 0.163 & 0.018 / 0.020 & \textbf{0.037} / \textbf{0.054} & 0.046 / 0.053\\
ablation 10 & 0.021 / 0.014 & \underline{0.007} / \underline{0.017} & 0.153 / 0.163 & 0.015 / \underline{0.020} & 0.045 / 0.060 & 0.048 / 0.055\\
\hline
Ground Truth & 0.000 & 0.001 & 0.021 & 0.000 & 0.002 & 0.005\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_ADE_min_FDE}
\subfloat[\ADE / \FDE]{
\label{table:eth_ucy_min_ADE_min_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{ADE}_{20} / \text{FDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.876 / 1.656 & 0.461 / 0.920 & 0.639 / 1.343 & 0.379 / 0.816 & 0.285 / 0.600 & 0.528 / 1.067\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.669 / 1.183 & 0.185 / 0.283 & 0.303 / 0.541 & 0.249 / 0.414 & 0.175 / 0.319 & 0.316 / 0.548\\
PECNet \cite{mangalam2020not} & 0.562 / 0.985 & 0.192 / 0.332 & 0.336 / 0.630 & 0.243 / 0.468 & 0.179 / 0.345 & 0.302 / 0.552\\
Y-Net no scene \cite{mangalam_goals_2020} & \textbf{0.318} / \textbf{0.377} & \underline{0.114} / \underline{0.169} & - / - & 0.213 / 0.394 & 0.147 / 0.263 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 0.398 / 0.571 & 0.123 / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448\\
Y-Net ped \cite{mangalam_goals_2020} & 0.404 / 0.602 & 0.154 / 0.281 & 14.144 / 27.618 & 0.254 / 0.381 & 0.174 / 0.324 & 3.026 / 5.841\\
Y-Net old \cite{mangalam_goals_2020} & \underline{0.323} / \underline{0.419} & 0.115 / \textbf{0.158} & - / - & 0.196 / 0.343 & 0.153 / 0.269 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 0.398 / 0.571 & 0.123 / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448\\
MemoNet \cite{Xu2022-ki} & 0.410 / 0.636 & \textbf{0.113} / 0.173 & \textbf{0.244} / \textbf{0.433} & \underline{0.184} / \underline{0.320} & \underline{0.143} / 0.248 & \textbf{0.219} / \textbf{0.362}\\
View Vertically \cite{Wong2022-kx} & 0.569 / 0.691 & 0.124 / 0.188 & 0.290 / 0.499 & 0.202 / 0.356 & 0.147 / 0.257 & 0.267 / 0.398\\
View Vertically w/ joint loss (Ours) & 0.662 / 0.833 & 0.130 / 0.196 & 0.316 / 0.546 & 0.216 / 0.364 & 0.151 / 0.261 & 0.295 / 0.440\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 0.144 / 0.221 & 0.297 / 0.522 & 0.215 / 0.390 & 0.147 / 0.257 & - / -\\
AgentFormer \cite{yuan_agentformer_2021} & 0.451 / 0.748 & 0.142 / 0.225 & \underline{0.254} / \underline{0.454} & \textbf{0.177} / \textbf{0.304} & \textbf{0.140} / \textbf{0.236} & \underline{0.233} / \underline{0.393}\\
\textbf{Joint AgentFormer (Ours)} & 0.473 / 0.792 & 0.135 / 0.212 & 0.285 / 0.505 & 0.189 / 0.321 & 0.144 / \underline{0.242} & 0.245 / 0.414\\
ablation 7.5 & 0.463 / 0.729 & 0.140 / 0.222 & 0.293 / 0.523 & 0.191 / 0.330 & 0.146 / 0.249 & 0.247 / 0.411\\
\textbf{Joint AgentFormer (old)} & 0.478 / 0.774 & 0.146 / 0.236 & 0.301 / 0.543 & 0.199 / 0.349 & 0.165 / 0.293 & 0.258 / 0.439\\
ablation 10 & 0.454 / 0.743 & 0.147 / 0.239 & 0.301 / 0.544 & 0.196 / 0.340 & 0.146 / 0.250 & 0.249 / 0.423\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_max_JADE_max_JFDE}
\subfloat[\max \text{JADE}_{20} / \text{JFDE}_{20}]{
\label{table:eth_ucy_max_JADE_max_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\max \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{1.559} / \textbf{3.308} & \underline{0.930} / \underline{2.040} & \textbf{0.855} / \textbf{1.804} & \textbf{0.863} / \textbf{2.028} & \textbf{0.752} / \textbf{1.660} & \textbf{0.992} / \textbf{2.168}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 2.092 / 4.451 & 1.259 / 2.714 & 0.911 / 2.007 & \underline{1.236} / \underline{2.746} & 0.936 / \underline{2.074} & 1.287 / 2.798\\
PECNet \cite{mangalam2020not} & \underline{1.762} / \underline{3.819} & 1.048 / 2.404 & \underline{0.888} / \underline{1.932} & 1.381 / 3.208 & \underline{0.916} / 2.171 & \underline{1.199} / \underline{2.707}\\
Y-Net no scene \cite{mangalam_goals_2020} & 2.354 / 4.887 & 1.019 / 2.315 & - / - & 1.750 / 3.913 & 1.035 / 2.330 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 2.420 / 4.985 & 1.024 / 2.265 & 1.245 / 2.837 & 2.217 / 4.830 & 1.490 / 3.388 & 1.679 / 3.661\\
Y-Net ped \cite{mangalam_goals_2020} & 2.271 / 4.696 & 1.268 / 2.770 & 58.218 / 127.453 & 1.550 / 3.366 & 1.114 / 2.433 & 12.884 / 28.144\\
Y-Net old \cite{mangalam_goals_2020} & 1.861 / 3.846 & \textbf{0.923} / \textbf{1.998} & - / - & 1.461 / 3.335 & 0.949 / 2.136 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 2.420 / 4.985 & 1.024 / 2.265 & 1.245 / 2.837 & 2.217 / 4.830 & 1.490 / 3.388 & 1.679 / 3.661\\
MemoNet \cite{Xu2022-ki} & 2.650 / 5.761 & 1.816 / 3.791 & 1.055 / 2.263 & 1.403 / 3.165 & 1.277 / 3.020 & 1.640 / 3.600\\
View Vertically \cite{Wong2022-kx} & 2.770 / 5.418 & 3.701 / 6.840 & 1.496 / 2.935 & 1.859 / 4.041 & 1.348 / 2.654 & 2.235 / 4.378\\
View Vertically w/ joint loss (Ours) & 4.488 / 7.995 & 1.968 / 2.744 & 1.476 / 2.749 & 4.791 / 6.851 & 1.243 / 2.463 & 2.793 / 4.560\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 4.008 / 5.637 & 4.406 / 6.896 & 1.826 / 3.866 & 1.295 / 2.568 & - / -\\
AgentFormer \cite{yuan_agentformer_2021} & 3.093 / 6.787 & 1.721 / 3.906 & 1.537 / 3.487 & 1.467 / 3.418 & 1.415 / 3.231 & 1.847 / 4.166\\
\textbf{Joint AgentFormer (Ours)} & 2.863 / 6.273 & 1.822 / 3.992 & 1.300 / 2.890 & 1.349 / 3.144 & 1.514 / 3.465 & 1.770 / 3.953\\
ablation 7.5 & 2.896 / 6.331 & 1.881 / 4.114 & 1.235 / 2.745 & 1.386 / 3.287 & 1.517 / 3.441 & 1.783 / 3.984\\
\textbf{Joint AgentFormer (old)} & 2.917 / 6.362 & 1.592 / 3.556 & 1.121 / 2.476 & 1.329 / 3.166 & 1.077 / 2.471 & 1.607 / 3.606\\
ablation 10 & 2.915 / 6.361 & 1.807 / 3.962 & 1.275 / 2.824 & 1.383 / 3.333 & 1.591 / 3.613 & 1.794 / 4.019\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_max_ADE_max_FDE}
\subfloat[\max \text{ADE}_{20} / \text{FDE}_{20}]{
\label{table:eth_ucy_max_ADE_max_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\max \text{ADE}_{20} / \text{FDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{1.567} / \textbf{3.372} & \textbf{1.007} / \textbf{2.218} & \textbf{0.952} / \textbf{2.000} & \textbf{0.882} / \textbf{2.055} & \textbf{0.795} / \textbf{1.781} & \textbf{1.041} / \textbf{2.285}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 2.134 / 4.597 & 1.562 / 3.375 & 1.683 / 3.716 & 1.609 / 3.553 & 1.459 / 3.201 & 1.689 / 3.688\\
PECNet \cite{mangalam2020not} & \underline{1.792} / \underline{3.944} & 1.261 / 2.875 & \underline{1.340} / \underline{2.976} & 1.789 / 4.118 & 1.301 / 3.078 & \underline{1.497} / \underline{3.398}\\
Y-Net no scene \cite{mangalam_goals_2020} & 3.086 / 6.501 & 1.388 / 3.209 & - / - & 2.337 / 5.194 & 1.542 / 3.521 & - / -\\
Y-Net ped no scene \cite{mangalam_goals_2020} & 2.733 / 5.599 & \underline{1.193} / \underline{2.647} & 1.910 / 4.326 & 2.773 / 5.979 & 2.001 / 4.550 & 2.122 / 4.620\\
Y-Net ped \cite{mangalam_goals_2020} & 2.460 / 5.094 & 1.434 / 3.131 & 84.622 / 185.765 & 1.948 / 4.265 & 1.411 / 3.074 & 18.375 / 40.266\\
Y-Net old \cite{mangalam_goals_2020} & 2.366 / 4.826 & 1.262 / 2.741 & - / - & 1.967 / 4.473 & 1.288 / 2.890 & - / -\\
Y-Net \cite{mangalam_goals_2020} & 2.733 / 5.599 & 1.193 / 2.647 & 1.910 / 4.326 & 2.773 / 5.979 & 2.001 / 4.550 & 2.122 / 4.620\\
MemoNet \cite{Xu2022-ki} & 2.971 / 6.439 & 2.356 / 4.896 & 1.914 / 4.070 & 1.879 / 4.192 & 1.925 / 4.630 & 2.209 / 4.845\\
View Vertically \cite{Wong2022-kx} & 2.920 / 5.636 & 3.999 / 7.369 & 1.998 / 3.818 & 2.003 / 4.354 & 1.640 / 3.132 & 2.512 / 4.862\\
View Vertically w/ joint loss (Ours) & 5.041 / 9.198 & 2.061 / 2.918 & 2.024 / 3.705 & 5.325 / 7.284 & 1.360 / 2.709 & 3.162 / 5.163\\
vv a 0.4,0.6 b 0.3,0.5,0.2 & - / - & 4.169 / 5.863 & 6.001 / 9.202 & 1.984 / 4.165 & 1.398 / 2.775 & - / -\\
AgentFormer \cite{yuan_agentformer_2021} & 3.311 / 7.274 & 1.793 / 4.051 & 1.932 / 4.396 & 1.559 / 3.614 & 1.611 / 3.675 & 2.041 / 4.602\\
\textbf{Joint AgentFormer (Ours)} & 3.007 / 6.658 & 1.856 / 4.108 & 1.642 / 3.664 & 1.347 / 3.129 & 1.639 / 3.772 & 1.898 / 4.266\\
ablation 7.5 & 3.042 / 6.723 & 1.885 / 4.147 & 1.635 / 3.643 & 1.401 / 3.304 & 1.618 / 3.717 & 1.916 / 4.307\\
\textbf{Joint AgentFormer (old)} & 3.072 / 6.774 & 1.546 / 3.495 & 1.454 / 3.247 & \underline{1.312} / \underline{3.106} & \underline{1.099} / \underline{2.552} & 1.697 / 3.835\\
ablation 10 & 3.079 / 6.787 & 1.790 / 3.964 & 1.651 / 3.680 & 1.401 / 3.354 & 1.726 / 3.944 & 1.930 / 4.346\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}

==> tables/temp-temp.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[tb]
\caption{}
\label{table:eth_ucy_min_JADE_min_JFDE}
\subfloat[\min \textit{JADE} / \min \textit{JFDE}]{
\label{table:eth_ucy_min_JADE_min_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.919 / 1.742 & 0.480 / 0.950 & 0.744 / 1.573 & 0.438 / 1.001 & 0.362 / 0.794 & 0.589 / 1.212\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.726 / 1.299 & 0.237 / 0.418 & 0.609 / 1.316 & 0.359 / 0.712 & 0.294 / 0.625 & 0.445 / 0.874\\
PECNet \cite{mangalam2020not} & 0.618 / 1.097 & 0.291 / 0.587 & 0.666 / 1.417 & 0.408 / 0.896 & 0.372 / 0.840 & 0.471 / 0.967\\
Y-Net \cite{mangalam_goals_2020} & 0.495 / \underline{0.781} & 0.205 / 0.386 & 0.695 / 1.559 & 0.487 / 1.045 & 0.492 / 1.101 & 0.475 / 0.974\\
MemoNet \cite{Xu2022-ki} & 0.499 / 0.859 & 0.222 / 0.416 & 0.686 / 1.466 & 0.349 / 0.723 & 0.385 / 0.864 & 0.428 / 0.866\\
View Vertically \cite{Wong2022-kx} & 0.561 / \textbf{0.776} & 0.196 / 0.332 & 0.654 / 1.307 & 0.328 / 0.654 & 0.298 / 0.602 & 0.408 / 0.734\\
View Vertically w/ joint loss (Ours) & 0.650 / 0.858 & \underline{0.187} / \textbf{0.315} & \textbf{0.578} / \textbf{1.202} & 0.333 / 0.635 & \underline{0.266} / \underline{0.547} & 0.403 / \underline{0.711}\\
AgentFormer \cite{yuan_agentformer_2021} & \textbf{0.482} / 0.794 & 0.237 / 0.456 & 0.622 / 1.310 & \underline{0.285} / \underline{0.564} & 0.296 / 0.624 & \underline{0.384} / 0.749\\
\textbf{Joint AgentFormer (Ours)} & \underline{0.485} / 0.798 & \textbf{0.186} / \underline{0.320} & \underline{0.590} / \underline{1.219} & \textbf{0.271} / \textbf{0.513} & \textbf{0.252} / \textbf{0.509} & \textbf{0.357} / \textbf{0.672}\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\subfloat[$CR_{JADE}$ / $CR_{mean}$]{
\label{table:eth_ucy_CR_of_best-JADE_sample_mean_collision_rate}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\text{CR}_{JADE} / \text{CR}_{mean} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.021 / 0.015 & 0.025 / 0.031 & \underline{0.165} / \underline{0.165} & 0.057 / 0.060 & 0.074 / 0.083 & 0.068 / 0.071\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.031 / 0.025 & 0.038 / 0.044 & 0.267 / 0.281 & 0.083 / 0.088 & 0.092 / 0.126 & 0.102 / 0.113\\
PECNet \cite{mangalam2020not} & \textbf{0.009} / 0.014 & 0.037 / 0.043 & 0.211 / 0.218 & 0.050 / 0.059 & 0.112 / 0.128 & 0.084 / 0.092\\
Y-Net \cite{mangalam_goals_2020} & 0.028 / 0.016 & 0.030 / 0.039 & 0.209 / 0.265 & 0.065 / 0.100 & 0.097 / 0.134 & 0.086 / 0.111\\
MemoNet \cite{Xu2022-ki} & 0.031 / 0.014 & 0.034 / 0.040 & 0.192 / 0.206 & 0.060 / 0.065 & 0.119 / 0.136 & 0.087 / 0.092\\
View Vertically \cite{Wong2022-kx} & 0.012 / 0.014 & 0.020 / 0.029 & 0.187 / 0.212 & 0.034 / 0.045 & 0.059 / 0.082 & 0.062 / 0.077\\
View Vertically w/ joint loss (Ours) & \underline{0.009} / \textbf{0.011} & 0.027 / 0.025 & 0.350 / 0.399 & 0.026 / 0.045 & 0.059 / 0.080 & 0.094 / 0.112\\
AgentFormer \cite{yuan_agentformer_2021} & 0.012 / 0.016 & \underline{0.019} / \underline{0.022} & 0.182 / 0.204 & \textbf{0.014} / \underline{0.021} & \underline{0.048} / \textbf{0.054} & \underline{0.055} / \underline{0.063}\\
\textbf{Joint AgentFormer (Ours)} & 0.017 / \underline{0.013} & \textbf{0.011} / \textbf{0.019} & \textbf{0.159} / \textbf{0.163} & \underline{0.015} / \textbf{0.021} & \textbf{0.041} / \underline{0.055} & \textbf{0.049} / \textbf{0.054}\\
\hline
Ground Truth & 0.000 & 0.001 & 0.021 & 0.000 & 0.002 & 0.005\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_KDE_NLL}
\subfloat[\min \textit{ADE} / \textit{FDE}]{
\label{table:eth_ucy_KDE_NLL}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$KDE NLL \downarrow$ ,  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & -2.958 & \underline{-2.611} & -1.682 & -2.230 & -1.674 & -2.231\\
Trajectron++ \cite{salzmann_trajectron_2021} & -2.795 & -2.380 & -1.633 & -2.249 & -1.711 & -2.154\\
PECNet \cite{mangalam2020not} & -2.837 & -2.427 & -1.605 & -2.429 & -1.781 & -2.216\\
Y-Net \cite{mangalam_goals_2020} & -3.102 & -2.347 & -1.557 & -2.556 & -1.769 & -2.266\\
MemoNet \cite{Xu2022-ki} & -3.040 & -2.467 & -1.676 & -2.389 & -1.918 & -2.298\\
View Vertically \cite{Wong2022-kx} & -3.429 & \textbf{-2.701} & \underline{-2.658} & \underline{-2.615} & \textbf{-2.125} & \underline{-2.706}\\
View Vertically w/ joint loss (Ours) & \textbf{-3.489} & -2.567 & \textbf{-2.741} & \textbf{-2.770} & \underline{-2.079} & \textbf{-2.729}\\
AgentFormer \cite{yuan_agentformer_2021} & -3.452 & -2.500 & -1.713 & -2.361 & -1.932 & -2.392\\
\textbf{Joint AgentFormer (Ours)} & \underline{-3.461} & -2.440 & -1.654 & -2.176 & -1.803 & -2.307\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_min_ADE_min_FDE}
\subfloat[\max \text{JADE}_{20} / \text{JFDE}_{20}]{
\label{table:eth_ucy_min_ADE_min_FDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\min \text{ADE}_{20} / \text{FDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & 0.876 / 1.656 & 0.461 / 0.920 & 0.639 / 1.343 & 0.379 / 0.816 & 0.285 / 0.600 & 0.528 / 1.067\\
Trajectron++ \cite{salzmann_trajectron_2021} & 0.669 / 1.183 & 0.185 / 0.283 & 0.303 / 0.541 & 0.249 / 0.414 & 0.175 / 0.319 & 0.316 / 0.548\\
PECNet \cite{mangalam2020not} & 0.562 / 0.985 & 0.192 / 0.332 & 0.336 / 0.630 & 0.243 / 0.468 & 0.179 / 0.345 & 0.302 / 0.552\\
Y-Net \cite{mangalam_goals_2020} & \textbf{0.398} / \textbf{0.571} & \underline{0.123} / 0.189 & 0.310 / 0.598 & 0.258 / 0.491 & 0.198 / 0.389 & 0.257 / 0.448\\
MemoNet \cite{Xu2022-ki} & \underline{0.410} / \underline{0.636} & \textbf{0.113} / \textbf{0.173} & \textbf{0.244} / \textbf{0.433} & \underline{0.184} / \underline{0.320} & 0.143 / 0.248 & \textbf{0.219} / \textbf{0.362}\\
View Vertically \cite{Wong2022-kx} & 0.569 / 0.691 & 0.124 / \underline{0.188} & 0.290 / 0.499 & 0.202 / 0.356 & 0.147 / 0.257 & 0.267 / 0.398\\
View Vertically w/ joint loss (Ours) & 0.697 / 0.805 & 0.129 / 0.197 & 0.306 / 0.551 & 0.219 / 0.360 & \underline{0.143} / 0.246 & 0.299 / 0.432\\
AgentFormer \cite{yuan_agentformer_2021} & 0.451 / 0.748 & 0.142 / 0.225 & \underline{0.254} / \underline{0.454} & \textbf{0.177} / \textbf{0.304} & \textbf{0.140} / \textbf{0.236} & \underline{0.233} / \underline{0.393}\\
\textbf{Joint AgentFormer (Ours)} & 0.473 / 0.792 & 0.135 / 0.212 & 0.285 / 0.505 & 0.189 / 0.321 & 0.144 / \underline{0.242} & 0.245 / 0.414\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\label{table:eth_ucy_max_JADE_max_JFDE}
\subfloat[\max \text{ADE}_{20} / \text{FDE}_{20}]{
\label{table:eth_ucy_max_JADE_max_JFDE}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccc|c}
\hline
\noalign{\smallskip}
 & \multicolumn{6}{c}{$\max \text{JADE}_{20} / \text{JFDE}_{20} \downarrow$  (m),  $K=20$ samples} \\
\cline{2-7}
\noalign{\smallskip} 
\;\;\;\;\;\;\;\; \text{Dataset \footnotesize(mean \# peds)} \rightarrow & ETH \footnotesize(1.4) & HOTEL \footnotesize(2.7) & UNIV \footnotesize(25.7) & ZARA1 \footnotesize(3.3) & ZARA2 \footnotesize(5.9) & ETH / UCY Avg.\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
S-GAN \cite{gupta_social_2018} & \textbf{1.559} / \textbf{3.308} & \textbf{0.930} / \textbf{2.040} & \textbf{0.855} / \textbf{1.804} & \textbf{0.863} / \textbf{2.028} & \textbf{0.752} / \textbf{1.660} & \textbf{0.992} / \textbf{2.168}\\
Trajectron++ \cite{salzmann_trajectron_2021} & 2.092 / 4.451 & 1.259 / 2.714 & 0.911 / 2.007 & \underline{1.236} / \underline{2.746} & 0.936 / \underline{2.074} & 1.287 / 2.798\\
PECNet \cite{mangalam2020not} & \underline{1.762} / \underline{3.819} & 1.048 / 2.404 & \underline{0.888} / \underline{1.932} & 1.381 / 3.208 & \underline{0.916} / 2.171 & \underline{1.199} / \underline{2.707}\\
Y-Net \cite{mangalam_goals_2020} & 2.420 / 4.985 & \underline{1.024} / \underline{2.265} & 1.245 / 2.837 & 2.217 / 4.830 & 1.490 / 3.388 & 1.679 / 3.661\\
MemoNet \cite{Xu2022-ki} & 2.650 / 5.761 & 1.816 / 3.791 & 1.055 / 2.263 & 1.403 / 3.165 & 1.277 / 3.020 & 1.640 / 3.600\\
View Vertically \cite{Wong2022-kx} & 2.770 / 5.418 & 3.701 / 6.840 & 1.496 / 2.935 & 1.859 / 4.041 & 1.348 / 2.654 & 2.235 / 4.378\\
View Vertically w/ joint loss (Ours) & 5.217 / 8.433 & 3.440 / 5.350 & 4.009 / 6.469 & 5.738 / 8.117 & 1.579 / 2.966 & 3.997 / 6.267\\
AgentFormer \cite{yuan_agentformer_2021} & 3.093 / 6.787 & 1.721 / 3.906 & 1.537 / 3.487 & 1.467 / 3.418 & 1.415 / 3.231 & 1.847 / 4.166\\
\textbf{Joint AgentFormer (Ours)} & 2.863 / 6.273 & 1.822 / 3.992 & 1.300 / 2.890 & 1.349 / 3.144 & 1.514 / 3.465 & 1.770 / 3.953\\

\hline
\end{tabular}
}  % end resizebox
}  % end subfloat



\end{table*}
